Future Architecture of the Interplanetary Internet

Fifty years after the Apollo program, space exploration has recently been regaining popularity thanks to missions with high media coverage. Future space exploration and space station missions will require specific networks to interconnect Earth with other objects and planets in the solar system. The interconnections of these networks form the core of an Interplanetary Internet (IPN). More specifically, we consider the IPN as the combination of physical infrastructure, network architecture, and technologies to provide communication and navigation services for missions and further applications. Compared to the current implementation of the Internet, nodes composing the core of the IPN are highly heterogeneous (base stations on planets, satellites etc.). Moreover, nodes are in constant motion over intersecting elliptical planes, which results in highly variable delays and even temporary unavailability of parts of the network. As such, an IPN has to overcome the challenges of conventional opportunistic networks, with much higher latency and jitter (from a couple of minutes to several days) and the additional constraint of long-term autonomous operations. In this paper, we highlight the challenges of IPN, demonstrate the elements to deploy within the areas of interest, and propose the technologies to handle deep space communication. We provide recommendations for an evolutionary IPN implementation, coherent with specific milestones of space exploration.

==> sec4_dtn.tex <==
\section{Delay Tolerant Networks (DTN)}
\label{sec:dtn}

The IPN Internet is an opportunistic network in which end-to-end latencies can reach up to a day, and jitter is measured in hours. 
As such, conventional Internet architectures based on the TCP/IP stack are not applicable. 
On the other hand, delay-tolerant architectures and protocols were designed to withstand the extreme constrains of the system. 
%\subsection{DTN Architecture}
% \begin{figure}[t]
%     \centering
%     \label{tcp_stack}
%     \includegraphics[width=9cm,height=9cm,keepaspectratio]{images/dtn_pr_stacks}
%     \caption{DTN vs TCP/IP protocol stacks}
%     \label{fig:dtntcpipstacks}
% \end{figure}
The first concepts of Delay Tolerant Networks (DTN)~\cite{fall2003delay,burleigh2003delay,fall2007delay} were originally proposed to cope with the characteristics of deep space communication (long delays, discontinuous network connectivity) before being extended to other domains.
The nodes of a DTN infrastructure are called DTN gateways and provide store-and-forward capabilities to handle the eventual link unavailabilities.
%which is subject to long delays and discontinuous network connectivity due to the motion of the planets and spacecraft.
%\todo[inline, color=green!40]{
%Due to the long distances between the planets and the motion of both the planets and spacecrafts, deep space communication is subject to long delays, discontinuous network connectivity. For these reasons, DTN architecture \cite{fall2003delay,burleigh2003delay,fall2007delay} has been developed to cope with these challenges.}
To cope with the long and variable latencies, DTN architectures insert
an overlay network protocol called \textbf{Bundling Protocol (BP)}, that provides end-to-end transmission between heterogeneous links. This overlay takes place on top of the transport protocol, ensuring compatibility with existing Internet infrastructures. At each point of the network, BP employs the transport protocol adapted to the transmission conditions.  BP can therefore operate over TCP~\cite{fall2011tcp,postel1981transmission} and UDP~\cite{postel1980user}, but also the Licklider Transport Protocol (LTP)~\cite{ramadas2008licklider,burleigh2008rfc,farrell2008licklider}, a  point-to-point transmission protocol for intermittent links with long propagation delays. Such characteristics makes it particularly adapted for interplanetary transmission, where the traditional TCP/IP paradigm cannot be applied. There are many DTN implementations for the Bundling Protocol (BP) that provides the store-and-forward capabilities required in deep space environment. In particular, Interplanetary Overlay Network (ION), and IRB-DTN were designed for deep space communication. 
% BP invokes the services of the underlying \textbf{Convergence Layer Protocol (CLP)} for each transport protocol to route the bundles along the path. CLP will in turn send and receive the bundles by using 'native' Internet protocols thanks to several Convergence Layer Adapters (CLA).


% This architecture is hardly compatible with the TCP/IP model at use on the Internet, mainly due to the high value and variance of latencies.
% Bundling protocols therefore provide an intercompatibility layer for interconnecting delay-tolerant applications and the Internet.




%; in the case of space communication, 
% here we refer to that Gateway Station, Relay Stations and DTN Nodes are the same 


% 
% This architecture is implemented in the Relay Nodes or so called \textbf{DTN Gateways}. These nodes in turn provide asynchronous messaging, using store-and-forward mechanisms into bundles. The relay node then forwards the bundle when the link to the next hop becomes available.
% By design, the overlay protocol cannot expect an end-to-end and must be adaptive to the conditions of the new communication environment.
% Burleigh et al. identified three principles of DTN architecture~\cite{burleigh2003delay}:
% \begin{itemize}
%   \item \textbf{A postal model of communication.} To take advantage of opportunistic networks such as the IPN, DTN applications should issue messages asynchronously. Furthermore, DTN application should not depend on prior negotiation, but instead integrate the negotiation messages into the bundles.
%   \item  \textbf{Tiered functionality.}  The existing routing protocols are more compatible and functionally efficient with the environment they already work in. Thus, DTN architecture should use all the capabilities of of the underlying protocols and performs any required additional functions.   
%   \item \textbf{Terseness.} Bandwidth is critical and precious. DTN protocols should therefore be less communicative.        
% \end{itemize} 



%\todo[inline]{how do we integrate DTN in a proper Internet setup? Any research made on this?}

%\todo[inline, color=green!40]{Please refer to Technologies Integration SmartSSR DTN Router}%
%\todo[inline]{This does not prevent to explain it in a small sentence here. For instance, you talk about protocol implementation in E}

%\subsection{DTN Bundling Protocols (BP)}

% \begin{figure}[t]
%     \centering
%     \label{bundle_forwarder}
%     \includegraphics[width=9cm,height=9cm,keepaspectratio]{images/BP_function}
%     \caption{example Implementation of Bundle Forwarder interaction with CLA and underlying protocols \cite{fall2008dtn}}
%     \label{fig:dtn_bp}
% \end{figure}

% Figure~\ref{fig:dtn_bp} shows the operation of the Bundling Protocol (BP)~\cite{scott2007bundle}. 
%BP operates as an overlay network above existing transport protocols.
% BP operates above an existing transport protocol, for instance, the traditional TCP~\cite{fall2011tcp,postel1981transmission} and UDP~\cite{postel1980user}, but also the Licklider Transport Protocol (LTP)~\cite{ramadas2008licklider,burleigh2008rfc,farrell2008licklider}. 
% LTP is a long-haul transmission point-to-point protocol for intermittent links with long propagation delays such as those encountered in deep space. It ensures the reliability of the transmission on the hop to hop basis.



% CLP employs a collection of protocol-specific convergence layer adapters (CLAs) necessary to carry bundles on top of each of the transport protocols. These CLAs enable for multiple CLP applications, including TCP-based CLP or TCPCL (BP/TCPCL/TCP/IP)~\cite{demmer2014delay}, UDP-based CLP  or UDPCL (BP/UDPCL/UDP/IP)~\cite{jero2014datagram}, TLP-based CLP or TLPCL (BP/TLPCL/TLP)~\cite{wang2011licklider}, Saratoga CLP~\cite{wood2007saratoga} and SpaceWire CLP~\cite{alfonzo2014development}. TCPCL and UDPCL mainly operate in terrestrial networks while the others focus on high stressed environment like deep-space communication.


% \subsection{DTN Protocol Implementations}


%In this section, we focus on three implementations that can be employed in the context of an IPN Internet.
% %\todo[inline]{Here, give a short sentence about why each protocol may be used in IPN. There is a bit too much descriptive information (we do not need that much), and too few implications towards our goal}
% \begin{itemize}
% \item \textbf{Interplanetary Overlay Network (ION) } is JPL's implementation of DTN architecture as described in Internet RFC 4838 to operate in Interplanetary environment. ION addresses the constrains enforced by the digital communication between IPN spacecraft and spaceflight control center\cite{burleigh2007ion}.
% It includes implementations of Bundling Protocol, Licklider Transmission Protocol, Interplanetary Communication Infrastructure (ICI) and other protocols that are intended to be usable in embedded environments including spacecraft flight computers\cite{ubuntu2007ion,sourceforge2007ion}.
% \item \textbf{DTN2} is the reference implementation. This implementation represents the components of the DTN architecture. It also provides a robust and flexible software framework for experimentation, extension, and real-world deployment.
% The core implementation is written in C++, which makes it particularly adapted to embedded systems.
% As the reference implementation, DTN2 includes a fairly comprehensive set of DTN functionalities, including the application api, support for custody, initial support for some of the DTN Security protocol, return receipts, a number of convergence layers including TCP, Bluetooth and LTP and an extensive collection of routing protocols~\cite{demmer2005dtn2,ohio2005dtn2}. 
% \item \textbf{IBR-DTN} is a modular and lightweight implementation of BP. Its main features are efficient resources usage and interoperability with DTN2\cite{doering2008ibr_dn,schildt2011ibr}.
% This implementation of BP %the bundle protocol RFC5050 
% is designed for embedded systems %like the RouterBoard 532A or Ubiquiti RouterStation Pro and can be used as framework for DTN applications. 
% with a modular architecture that allows to easily develop functionalities~\cite{jmorgenroth2008ibrdtn,github2008ibrdtn}.
% %\item \textbf{JDTN} is Java-based implementation of Delay Tolerant Networking (DTN). It runs on any platform that supports Java, including Android\cite{jdtn}.
% \end{itemize}
% The Interplanetary Overlay Network (ION) is a solid candidate as it has been specifically designed for space communication. 
% However, DTN-2, the reference implementation, is also a good candidate due to its versatility and especially its compatibility with TCP. Finally, IRB-DTN is a lightweight solution, adapted to resource constrained systems such as satellites. 
% It is also compatible with DTN-2, which can be implemented on ground stations. %Finally, JDTN is slightly out of the scope of our study as it tends to target the end users rather than the core network.





